Are Small Language Models Ready to Compete with Large Language Models for Practical Applications?

The rapid rise of Language Models (LMs) has expanded their use in several applications. Yet, due to constraints of model size, associated cost, or proprietary restrictions, utilizing state-of-the-art (SOTA) LLMs is not always feasible. With open, smaller LMs emerging, more applications can leverage their capabilities, but selecting the right LM can be challenging as smaller LMs do not perform well universally. This work tries to bridge this gap by proposing a framework to experimentally evaluate small, open LMs in practical settings through measuring semantic correctness of outputs across three practical aspects: task types, application domains, and reasoning types, using diverse prompt styles. It also conducts an in-depth comparison of 10 small, open LMs to identify the best LM and prompt style depending on specific application requirements using the proposed framework. We also show that if selected appropriately, they can outperform SOTA LLMs like DeepSeek-v2, GPT-4o, GPT-4o-mini, Gemini-1.5-Pro, and even compete with GPT-4o.

==> paper_sections/main/introduction.tex <==
\section{Introduction}

The field of NLP has advanced significantly with the rise of Language Models (LMs). Rapid development of LMs~\cite{gpt3,llama2,falcon,gemma,deepseekv2} has expanded their use across numerous types like Title Generation~\citep{keles-bayrakli-2024-llama-2}, Data Exploration~\citep{ma-etal-2023-insightpilot}, Dialogue act recognition~\citep{qiang-etal-2024-prompt}; domains like Economics \& Finance~\citep{rajpoot-etal-2024-adapting-llm, yu-etal-2023-harnessing}, Politics~\citep{feng-etal-2023-pretraining}, Nutrition \& Food~\citep{yang2024chatdiet}, News~\citep{kuila-sarkar-2024-deciphering}; and reasoning types~\citep{huang-chang-2023-towards} like ANALOGICAL~\citep{wijesiriwardene-etal-2023-analogical} and Multi-hop~\citep{pan-etal-2021-unsupervised} reasoning.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{assets/descriptive/inst_eval_paper-outline-2.drawio.pdf}
    \caption{Outline of this work: Performance analysis of open, small-scale LMs and best prompt style for task types, application domains, and reasoning types.}
    \label{fig:outline}
\end{figure}

Initially, LMs were relatively weak like GPT-2~\citep{gpt2}, too large in size like GPT-3~\citep{gpt3}, expensive like GPT-4~\citep{gpt4}, and/or closed and accessible only via APIs. These pose challenges of accessibility, computational resource limitations~\citep{ding2024efficiency}, costs~\citep{jimenez-gutierrez-etal-2022-thinking} (GPT-4 Turbo charges \$10/1M input, \$30/1M output tokens), data privacy, inflexibility of customization, and so on. However, there has been recent rise in competitive LMs which are relatively small and openly available. These properties remove the aforementioned limitations, and provide additional benefits like on-device usage, faster inference time, easier compliance and security management.

But do these smaller LMs fit every use case like the SOTA LLMs? They vary a lot in terms of training data, pre-training strategies, and architectural decisions. Further, utilization strategies like zero-shot usage, customizing pre-trained models (e.g., fine-tuning~\citep{mosbach-etal-2023-shot}), using in-context learning~\citep{icl,icl_survey}, prompt engineering~\citep{gpt3} can differ with varying need. Writing helpful prompts also requires time and domain expertise. For someone to use these small, open LMs, they need to conduct their analysis with constraints of time, money, computational resources is a complicated task, and identify the LMs fit for their use. Technical reports of some LMs~\citep{gemma,gemma2} report performance on different benchmarks, but they are more theoretical than in a practical usage setting. Therefore, there is a need for a comprehensive evaluation of these LMs and determining their capabilities for different use cases in different practical applications and determining if one can use them instead of SOTA LLMs within tolerable levels of performance degradation.

To bridge this gap, we perform this extensive, in-depth experimental analysis with 10 openly available LMs between 1.7B--11B parameters. We also vary prompt styles by using chat-style task definitions, in-context examples that are closer to how users interact with LMs, and evaluate them across three aspects -- task types, application domains and reasoning types, which can be considered as three different ways of categorizing an application area aiming to use LMs. We propose a schema by selecting 12, 12, and 10 entities from each aspect respectively in English language covering a broad range of areas, and group similar entities. For example, in application domains, we group `Social Media' and `News' in `Media and Entertainment'. This three-tier structure (aspect, group, entity) allows finding patterns in capabilities of LMs at multiple levels, along different aspects. 

A recent work~\citep{lora_land} dives into efficacy of LoRA~\citep{lora} fine-tuning of smaller LMs, but uses static prompts, and limits to varying task types only. Further, usage strategy of LMs can significantly vary -- fine-tuning~\citep{mosbach-etal-2023-shot}, PEFT~\citep{peft_survey}, multi-stage pipeline based, or directly with/without prompt engineering due to lack of sufficient data, resources, or need for customization. Hence, we consider semantic correctness of outputs as a measure of LMs' innate ability, and evaluate 5 pre-trained and 5 instruction-tuned (IT)~\citep{instructGPT} LMs out-of-the-box with 8 prompt styles. We show that scale can be countered with careful selection of small, open LMs, which can enable matching and outperforming models like GPT-4o-mini, GPT-4o~\citep{gpt4o}, DeepSeek-v2~\citep{deepseekv2} and Gemini-1.5-Pro~\citep{gemini-1.5} for practical applications. Our proposed framework enables this analysis and identifies patterns in strengths and weaknesses at 3 hierarchical levels.

In this work, we aim to address these research questions: \textbf{(i)} Can small, open LMs compete with large, proprietary LMs in practical usage? \textbf{(ii)} What can be an exhaustive evaluation framework to conduct this analysis? \textbf{(iii)} For different application needs, how do current best small, open LMs perform in comparison, and which LM is the best choice? \textbf{(iv)} What type of prompt style should be used to extract best results from these LMs? 

Consistent with Figure~\ref{fig:outline}, we make the following \textbf{key contributions}: 

{(i)} Propose a three-tier evaluation framework to analyze performance of LMs for different \textit{task types}, \textit{application domains} and \textit{reasoning types}.

{(ii)} Conduct an in-depth experimental analysis of semantic correctness of outputs of 10 open, small LMs in 2B--11B size based on the framework.

{(iii)} Show that appropriate selection of open, small LMs can lead to outperforming SOTA LLMs like GPT-4o-mini, Gemini-1.5-Pro, and competing with GPT-4o.

{(iv)} Compare the performance of LMs with eight prompt styles and recommend the best alternative.

